Bond formation insights into the Diels-Alder reaction: A bond perception and self-interaction perspective

The behavior of electrons during bond formation and breaking cannot commonly be accessed from experiments. Thus, bond perception is often based on chemical intuition or rule-based algorithms. Utilizing computational chemistry methods, we present intrinsic bond descriptors for the Diels-Alder reaction, allowing for an automatic bond perception. We show that these bond descriptors are available from localized orbitals and self-interaction correction calculations, e.g., from Fermi-orbital descriptors. The proposed descriptors allow a sparse, simple, and educational inspection of the Diels-Alder reaction from an electronic perspective. We demonstrate that bond descriptors deliver a simple visual representation of the concerted bond formation and bond breaking, which agrees with Lewis' theory of bonding.

==> acro.style.abbrev.code.tex <==
% !TEX root = main.tex
\AcroStyle{abbrev}

\DeclareAcronym{lda}{
   	short = LDA,
   	long  = local density approximation
}
\DeclareAcronym{gga}{
   	short = GGA,
   	long  = generalized gradient approximation
}
\DeclareAcronym{mgga}{
   	short = meta-GGA,
   	long  = meta-GGA,
    first-style = short
}
\DeclareAcronym{dft}{
   	short = DFT,
   	long  = density functional theory
}
\DeclareAcronym{sic}{
	short = SIC,
	long  = self-interaction correction
}
\DeclareAcronym{sie}{
	short = SIE,
	long  = self-interaction error
}
\DeclareAcronym{flo}{
	short = FLO,
	long  = Fermi-L\"owdin orbital
}
\DeclareAcronym{flosic}{
	short = FLO-SIC,
	long  = FLO-SIC,
    first-style = short
}
\DeclareAcronym{fo}{
	short = FO,
	long  = Fermi orbital
}
\DeclareAcronym{fod}{
	short = FOD,
	long  = Fermi-orbital descriptor
}
\DeclareAcronym{scf}{
	short = SCF,
	long  = self-consistent field
}
\DeclareAcronym{ks}{
	short = KS,
	long  = Kohn-Sham
}
\DeclareAcronym{spw}{
	short = SPW92,
	long  = SPW92
}
\DeclareAcronym{kso}{
	short = KSO,
	long  = Kohn-Sham orbital
}
\DeclareAcronym{pz}{
	short = PZ,
	long  = Perdew-Zunger
}
\DeclareAcronym{pzsic}{
	short = PZ-SIC,
	long  = PZ-SIC,
    first-style = short
}
\DeclareAcronym{gto}{
	short = GTO,
	long  = Gaussian-type orbital
}
\DeclareAcronym{ts}{
	short = TS,
	long  = transition state
}
\DeclareAcronym{fb}{
	short = FB,
	long  = Foster-Boys
}
\DeclareAcronym{er}{
	short = ER,
	long  = Edmiston-Ruedenberg
}
\DeclareAcronym{pm}{
	short = PM,
	long  = Pipek-Mezey
}
\DeclareAcronym{ibo}{
	short = IBO,
	long  = intrinsic bond orbital
}
\DeclareAcronym{neb}{
	short = NEB,
	long  = nudged elastic bands
}
\DeclareAcronym{hei}{
	short = HEI,
	long  = highest energy image
}
\DeclareAcronym{mep}{
	short = MEP,
	long  = minimum energy path
}
\DeclareAcronym{uff}{
	short = UFF,
	long  = universal force field
}
\DeclareAcronym{ciah}{
	short = CIAH,
	long  = co-iterative augmented Hessian
}
\DeclareAcronym{abp}{
	short = ABP,
	long  = associated bond point
}
\DeclareAcronym{lt}{
	short = LT,
	long  = Lewis theory
}
\DeclareAcronym{aim}{
	short = AIM,
	long  = atoms in molecules
}
\DeclareAcronym{dfa}{
	short = DFA,
	long  = density functional approximation
}
\DeclareAcronym{foss}{
    short = FOSS,
    long = free and open-source software 
}
\DeclareAcronym{elf}{
    short = ELF,
    long = electron localization function
}
\DeclareAcronym{rfo}{
    short = RFO,
    long = rational function optimization
}
\DeclareAcronym{rsrfo}{
    short = RS-RFO,
    long =RS-RFO
}
\DeclareAcronym{rsirfo}{
    short = RS-I-RFO,
    long = RS-I-RFO
}
\DeclareAcronym{oee}{
    short = OEE,
    long = one-electron error
}
\DeclareAcronym{me}{
    short = ME,
    long = mean error,
    first-style = long-short
}
\DeclareAcronym{mae}{
    short = MAE,
    long = mean absolute error,
    first-style = long-short
}
\DeclareAcronym{mm}{
    short = MM,
    long = molecular mechanics,
    first-style = long-short
}
